Deep Direct Discriminative Decoders for High-dimensional Time-series Data Analysis

The state-space models (SSMs) are widely utilized in the analysis of time-series data. SSMs rely on an explicit definition of the state and observation processes. Characterizing these processes is not always easy and becomes a modeling challenge when the dimension of observed data grows or the observed data distribution deviates from the normal distribution. Here, we propose a new formulation of SSM for high-dimensional observation processes. We call this solution the deep direct discriminative decoder (D4). The D4 brings deep neural networks' expressiveness and scalability to the SSM formulation letting us build a novel solution that efficiently estimates the underlying state processes through high-dimensional observation signal. We demonstrate the D4 solutions in simulated and real data such as Lorenz attractors, Langevin dynamics, random walk dynamics, and rat hippocampus spiking neural data and show that the D4 performs better than traditional SSMs and RNNs. The D4 can be applied to a broader class of time-series data where the connection between high-dimensional observation and the underlying latent process is hard to characterize.

==> temp_intro.tex <==
%New advances in SSMs focused on circumventing this problem by increasing the dimension of the state variables, characterizing the observation conditional distribution becomes easy given a large set of state variables \cite{zoltowski2020general,linderman2017bayesian,glaser2020machine}. Although this approach increases the expressive power of SSMs, we lose the interpretability of the expanded state variables, given the extra state variable might not represent the temporal dynamics of the underlying physical or biological systems. In addition, identifying the optimal number of the state dimension is computationally intractable, and the proposed solutions lack a mechanism for identifying the number of states.\\
%Most recently, discriminative models such as deep neural networks (DNNs) and recurrent neural networks (RNNs) \cite{burkhart2020discriminative, krishnan2015deep, rezaei2018comparison,Rezaei_neco_a_01491, glaser2020recurrent} 
 %{\color{red} (Here we focused on discriminative properties of DNNs, although in another context it also can be seen as generative models)} are introduced to SSM for increasing its scalability in the analysis of high dimensional data. A modeling concern with these solutions is that the DNN expressive power is not efficiently embedded in their solutions; as a result, they will not necessarily address the challenges of characterizing high-dimensional observation \cite{gao2016linear,johnson2016structured, krishnan2015deep, archer2015black}. For instance, the discriminative Kalman filters (DKFs) \cite{burkhart2020discriminative} and direct discriminative decoders (DDD) \cite{Rezaei_neco_a_01491} use a simple discriminative model, such as a linear model with an additive Gaussian noise or the history of observed signals is discarded in the estimation of the state. In other solutions like the deep Kalman filter (Deep-KF)\cite{krishnan2015deep}, the linear observation and state transition processes are replaced with DNNs \cite{krishnan2015deep,rangapuram2018deep} and mainly ignore temporal dynamics of the underlying biological or physical systems. This modeling assumption is prohibitive when a proper prior is available for the state dynamics, or the interpretability of the inferred state is of interest.\\
%A critical advantage of SMMs is their explicit definition of the state dynamics and observation processes that allow information carried by the state and observation to be optimally combined to infer the underlying latent dynamics. In the meantime, the advantage of the DNNs and RNNs is expressive power and scalability. The deep direct discriminative decoder (D4) solution proposed here leverages both SSM and DNN advantages in characterizing observed signals and inference of the underlying dynamics. The D4 incorporates a state transition process like the way is being utilized in SSMs and utilizes DNN or RNNs to augment the conditional distribution of observation by a discriminative process.



%In contrast to the previous solutions, our discriminative process can maintain DNN's expressiveness as it optimally combines the current and history of the observation in its estimation of the underlying state. We argue that the D4 will not only address scalability issues we face in SSMs for high-dimensional time-series data but also will reach a high level of accuracy in the estimation of state dynamics. {\color{red} We tested D4 on simulation and real datasets, where the D4 outperformed traditional DNN and SSM models in squared error (MSE), mean absolute error (MAE) performance measure (see Figure \ref{fig:D4_Maze_obs_perf_comp})}. The D4 applications are broader and can be applied to different modalities of time-series data without constraints on the modality or distribution of observed data. We argue D4 solution facilitates the analysis of high-dimensional data where the connection between the high-dimensional observation and the underlying state process needs to be interpretable.
